On a fractional system of NLS-KDV equations with Hardy potentials

In this article, our main concern is to study the existence of bound and ground state solutions for the following fractional system of nonlinear Schr\"odinger-Korteweg-De Vries (NLS-KdV, in short) equations with Hardy potentials: \begin{equation*} \left\{ \begin{aligned} (-\Delta)^{s_{1}} u - \lambda_{1} \frac{u}{|x|^{2s_{1}}} - u^{2_{s_{1}}^{*}-1} &= 2\nu h(x) u^{}v^{} & \quad \mbox{in} ~ \mathbb{R}^{N}, (-\Delta)^{s_{2}} v - \lambda_{2} \frac{v}{|x|^{2s_{2}}} - v^{2_{s_{2}}^{*}-1} &= \nu h(x) u^{2} & \quad \mbox{in} ~ \mathbb{R}^{N}, u,v >0 \quad \mbox{in} ~ \mathbb{R}^{N} \setminus \{0\}, \end{aligned} \right. \end{equation*} where $s_{1},s_{2} \in (0,1)~\text{and}~\lambda_{i}\in (0, \Lambda_{N,s_{i}})$ with $\Lambda_{N,s_{i}} = 2 \pi^{N/2} \frac{\Gamma^{2}(\frac{N+2s_i}{4}) \Gamma(\frac{N+2s_i}{2})}{\Gamma^{2}(\frac{N-2s_i}{4}) ~|\Gamma(-s_{i})|}, (i=1,2)$. By imposing certain assumptions on the parameter $\nu$ and on the function $h$, we obtain ground-state solutions using the concentration-compactness principle and the mountain-pass theorem.

==> Preamble.tex <==
\usepackage{multirow}
\usepackage{eqnarray,amsmath}
\usepackage{amsmath,graphicx,subfigure}
\usepackage{amssymb,amsfonts,amsthm,anysize,url}
\usepackage{caption}
\usepackage{mathrsfs}
\usepackage{graphicx}
\usepackage{xcolor}
\usepackage[colorlinks=true,linkcolor=blue]{hyperref}%
\newcounter{saveenumi}
\newcommand{\seti}{\setcounter{saveenumi}{\value{enumi}}}
\newcommand{\conti}{\setcounter{enumi}{\value{saveenumi}}}
% \newtheorem{definition}{Definition}  
% \newtheorem{remarks}{Remarks}
% \newtheorem{lemma}{Lemma}
% \newtheorem{proposition}{Proposition}
% \newtheorem{corollary}{Corollary}
% \newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}[definition]{Theorem}
\newtheorem{example}[definition]{Example}
\newtheorem{corollary}[definition]{Corollary}
\newtheorem{remark}[definition]{Remark}
\newtheorem{proposition}[definition]{Proposition}
\newtheorem{lem}[definition]{Lemma}
% \newtheorem{defn}[definition]{Definition}
\newtheorem{lemma}[definition]{Lemma}
\newtheorem{result}[definition]{Result}
\numberwithin{equation}{section}

==> prelim1.tex <==
\section{Preliminaries and functional setting}\label{S2}

In this section, we give an appropriate variational setting for the system \eqref{main problem}. First, we define the energy functional $J_\nu$ associated with the system \eqref{main problem} given as
\begin{align} \label{energy functional}
\begin{split}
    J_{\nu}(u,v) &= \frac{1}{2} \iint_{\mathbb{R}^{2N}} \frac{|u(x)-u(y)|^{2}}{|x-y|^{N+2s_{1}}} \mathrm{d}x \mathrm{d}y + \frac{1}{2} \iint_{\mathbb{R}^{2N}} \frac{|v(x)-v(y)|^{2}}{|x-y|^{N+2s_{2}}} \mathrm{d}x \mathrm{d}y -  \frac{\lambda_{1}}{2} \int_{\mathbb{R}^{N}} \frac{u^{2}~~}{|x|^{2s_{1}}}\mathrm{d}x\\
    &~~~~~  - \frac{\lambda_{2}}{2} \int_{\mathbb{R}^{N}} \frac{v^{2}~~}{|x|^{2s_{2}}}\mathrm{d}x - \frac{1}{2_{s_{1}}^{*}}\int_{\mathbb{R}^{N}} |u|^{2_{s_{1}}^{*}}\mathrm{d}x  -\frac{1}{2_{s_{2}}^{*}}\int_{\mathbb{R}^{N}} |v|^{2_{s_{2}}^{*}}\mathrm{d}x - \nu \int_{\mathbb{R}^{N}}h(x) u^{2} v  \, \mathrm{d}x,
\end{split}
\end{align} 
defined on the product space $\mathbb{D} = \mathcal{D}^{s_{1},2}(\mathbb{R}^{N}) \times \mathcal{D}^{s_{2},2}(\mathbb{R}^{N})$. The space $\mathcal{D}^{s_i,2}(\mathbb{R}^{N}),~( i=1,2)$ is the closure of $C_{0}^{\infty}(\mathbb{R}^{N})$ with respect to the Gagliardo seminorm
\[ \|u\|_{s_i} := \bigg( \iint_{\mathbb{R}^{2N}} \frac{|u(x)-u(y)|^{2}}{|x-y|^{N+2s_{i}}}\,\mathrm{d}x\mathrm{d}y  \bigg)^{\frac{1}{2}},~~\text{for}~i=1,2.\]
We refer to the articles \cite{Brasco2021characterisation,Brasco2019note} by Brasco et al. for more details about the space $\mathcal{D}^{s_i,2}(\mathbb{R}^{N}),~( i=1,2)$. Further, we endow the following norm with the product space $\mathbb{D}$ given by
$$ \|(u,v)\|^{2}_{\mathbb{D}} = \|u\|_{\lambda_{1}, s_{1}}^{2} + \|v\|_{\lambda_{2}, s_{2}}^{2},  $$
where
$$ \|u\|_{\lambda_i, s_i}^{2} = \iint_{\mathbb{R}^{2N}} \frac{|u(x)-u(y)|^{2}}{|x-y|^{N+2s_{i}}}\,\mathrm{d}x\mathrm{d}y - \lambda_i \int_{\mathbb{R}^{N}}\frac{u^{2}}{|x|^{2s_i}}\,\mathrm{d}x,~\text{for}~i =1,2. $$
The above norm is well defined due to the fractional Hardy inequality \cite[Theorem 1.1]{Frank2008} given by
\begin{equation} \label{fractional Hardy inequality}
    \Lambda_{N,s_i} \int_{\mathbb{R}^{N}}\frac{{u^{2}}}{|x|^{2s_i}}\mathrm{d}x \leq \iint_{\mathbb{R}^{2N}} \frac{|u(x)-u(y)|^{2}}{|x-y|^{N+2s_{i}}} \mathrm{d}x\mathrm{d}y, ~\text{for}~i =1,2.
\end{equation}
where $\Lambda_{N,s_{i}} = 2 \pi^{N/2} \frac{\Gamma^{2}(\frac{N+2s_i}{4}) \Gamma(\frac{N+2s_i}{2})}{\Gamma^{2}(\frac{N-2s_i}{4}) ~|\Gamma(-s_{i})|}, (i=1,2)$ is the sharp constant for the inequality \eqref{fractional Hardy inequality}. We can note that the norms $\|\cdot\|_{\lambda_i,s_i}$ and $\|\cdot\|_{s_i}$ for any $\lambda_i \in (0, \Lambda_{N,s_i})~\text{with}~ i=1,2$ are equivalent due to the Hardy’s inequality \eqref{fractional Hardy inequality}. 

Let us recall that the solutions of \eqref{single problem} arise as minimizers $z^{\lambda_i}_{\mu,s_i}~(i=1,2)$ of the Rayleigh quotient given by (see \cite{Dipierro2016})
\begin{equation}\label{S lambda}
    S(\lambda_i) := \inf\limits_{u \in \mathcal{D}^{s_i,2}(\mathbb{R}^{N}), u \not\equiv 0} \frac{\|u\|_{\lambda_{i},s_i}^{2}}{\|u\|_{2_{s_i}^{*}}^{2}~~} = \frac{\|z^{\lambda_i}_{\mu,s_i}\|_{\lambda_{i},s_i}^{2}}{\|z^{\lambda_i}_{\mu,s_i}\|_{2_{s_i}^{*}}^{2}~~}, (i=1,2).
\end{equation}
Moreover, we have
\begin{equation} \label{extremal value at norms}
  \|z^{\lambda_i}_{\mu,s_i}\|_{\lambda_{i},s_i}^{2} = \|z^{\lambda_i}_{\mu,s_i}\|_{2_{s_i}^{*}}^{2_{s_i}^{*}} = S^{\frac{N}{2s_i}}(\lambda_i),~\text{for}~i=1,2. 
\end{equation}
If $\lambda_i =0$ for $i=1,2$, then $S(\lambda_i)=S_i$ which is known to be achieved by the extremal functions of the type $C(N,s_i)(1+|x|^2)^{-\frac{N-2s_i}{2}}$ (see \cite{Lieb2002sharp}), where $C(N,s_i)$ is a positive constant depending on $N$ and $s_i$ only. We write $S_1=S_2=S$ when $s_1=s_2.$ Let us re-write the functional $J_{\nu}(u,v)$ as 
\begin{equation}
    J_{\nu}(u,v) = J_{\lambda_1}(u_{}) + J_{\lambda_2}(v_{}) - \nu \int_{\mathbb{R}^{N}}h(x) u^{2} v 
 \,\mathrm{d}x,
\end{equation}
where
\begin{align} \label{value of functional componentwise}
    J_{\lambda_i}(u_{}) = \frac{1}{2} \iint_{\mathbb{R}^{2N}} \frac{|u(x)-u(y)|^{2}}{|x-y|^{N+2s_{i}}} \,\mathrm{d}x\mathrm{d}y  -  \frac{\lambda_{i}}{2} \int_{\mathbb{R}^{N}} \frac{u^{2}}{|x|^{2s_{i}}}\,\mathrm{d}x  - \frac{1}{2_{s_{i}}^{*}}\int_{\mathbb{R}^{N}} |u|^{2_{s_{i}}^{*}}\,\mathrm{d}x,~ \text{for}~i=1,2.
\end{align}
The functional $J_\nu$ is well-defined and is $C^2$ on the product space $\mathbb{D}$. In the following, we are going to prove that the functional  $J_{\nu}$ is  $C^1$ first and a similar argument will be followed for $C^2$ as well.  \\
\textbf{(a). The functional $J_\nu$ is well-defined on $\mathbb{D}=\mathcal{D}^{s_{1},2}(\mathbb{R}^{N}) \times \mathcal{D}^{s_{2},2}(\mathbb{R}^{N})$ :}
It follows that
\begin{align} \label{f2}
    |J_{\nu}(u,v)| & \leq \frac{1}{2} \|(u,v)\|_{\mathbb{D}}^2 + \frac{1}{2_{s_{1}}^{*}} \|u\|_{2_{s_{1}}^{*}}^{2_{s_{1}}^{*}}  +\frac{1}{2_{s_{2}}^{*}}\|v\|_{2_{s_{2}}^{*}}^{2_{s_{2}}^{*}} + \nu \int_{\mathbb{R}^{N}}h(x)|u|^{2}|v|^{}\, \mathrm{d}x.
\end{align} 
The first term in the above inequality is finite as it is a norm on the product space $\mathbb{D}$. 
We recall the Sobolev embeddings
\begin{equation} \label{embeddings}
%\begin{split}
    S(\lambda_i) \|u\|_{2_{s_i}^{*}}^{2} \leq \|u\|_{\lambda_{1},s_i}^{2}, \text{ for } i=1,2.
%\end{split}
\end{equation} 
By using the above embeddings, it immediately follows that the second and third terms in \eqref{f2} are finite. Now just we need to check the finiteness of the last term in \eqref{f2}. Let us denote the integral as $I= \int_{\mathbb{R}^{N}}h(x)|u|^{2}|v|^{}\, \mathrm{d}x$. It is given $N \leq \min\{6{s_1}, 6s_2 \}$, and the function $h$ is positive with $h \in L^{1}(\mathbb{R}^N) \cap L^{\infty}(\mathbb{R}^N)$.\\
\textbf{Case 1.}  $N < \min\{6{s_1}, 6s_2\}$\\
If $s_1 \geq s_2$, then $2_{s_1}^{*}\geq 2_{s_2}^{*}$ which further implies $\frac{2}{2_{s_1}^{*}} + \frac{1}{2_{s_2}^{*}} \leq \frac{3}{2_{s_2}^{*}} <1$. By symmetry, the condition $s_2 \geq s_1$ also implies $\frac{2}{2_{s_1}^{*}} + \frac{1}{2_{s_2}^{*}} <1$. Now we have
\[ I = \int_{\mathbb{R}^{N}}h(x)|u|^{2}|v|^{}\, \mathrm{d}x = \int_{\mathbb{R}^{N}}(h(x))^{{1-\frac{2}{2_{s_1}^{*}}} - \frac{1}{2_{s_2}^{*}}} (h(x)^{\frac{2}{2_{s_1}^{*}}}|u|^{2}) (h(x)^{\frac{1}{2_{s_2}^{*}}}|v|)\, \mathrm{d}x \]
Since the continuous embedding $\mathcal{D}^{s_i,2}(\mathbb{R}^{N}) \hookrightarrow L^{2_{s_i}^{*}}(\mathbb{R}^{N}),~(i=1,2)$ and $h \in L^{\infty}(\mathbb{R}^{N})$, it follows that $h(x)^{\frac{2}{2_{s_1}^{*}}} |u|^{2} \in L^{\frac{2_{s_1}^{*}}{2}}(\mathbb{R}^{N})$ and similarly $h(x)^{\frac{1}{2_{s_2}^{*}}} |v| \in L^{2_{s_2}^{*}}(\mathbb{R}^{N})$. Also, the assumption $h \in L^{1}({\mathbb{R}^N})$ implies $\displaystyle (h(x))^{{1-\frac{2}{2_{s_1}^{*}}} - \frac{1}{2_{s_2}^{*}}} \in L^{\frac{1}{{1-\frac{2}{2_{s_1}^{*}}} - \frac{1}{2_{s_2}^{*}}}}({\mathbb{R}^N})$.\\

We denote by $p=\frac{2_{s_1}^{*}}{2},~ q= 2_{s_2}^{*}$ and $r = \frac{1}{{1-\frac{2}{2_{s_1}^{*}}} - \frac{1}{2_{s_2}^{*}}}$. Since $\frac{1}{p} + \frac{1}{q} + \frac{1}{r} =1$, by generalized H\"{o}lder's inequality it follows that
\begin{align*}
    I &\leq \bigg(\int_{\mathbb{R}^{N}}h(x)\, \mathrm{d}x \bigg)^{1/r} \bigg( \int_{\mathbb{R}^{N}}h(x)|u|^{2_{s_1}^{*}}\, \mathrm{d}x \bigg)^{1/p} \bigg(\int_{\mathbb{R}^{N}}h(x)|v|^{2_{s_2}^{*}}\, \mathrm{d}x \bigg)^{1/q}\\
    &\leq \|h\|_{1}^{1/r} \|h\|_{\infty}^{1/p + 1/q}\bigg( \int_{\mathbb{R}^{N}} |u|^{2_{s_1}^{*}}\, \mathrm{d}x \bigg)^{1/p} \bigg(\int_{\mathbb{R}^{N}} |v|^{2_{s_2}^{*}}\, \mathrm{d}x \bigg)^{1/q}.
\end{align*}
Since the right side integrals are finite due to the Sobolev embeddings given in \eqref{embeddings} and $h \in L^{1}({\mathbb{R}^{N}}) \cap L^{\infty}({\mathbb{R}^{N}})$, the integral $I$ is well-defined on the product space $\mathbb{D}$.\\
\textbf{Case 2.}  When $N = \min\{6s_1, 6s_2\}.$\\
For $s_1 \geq s_2$ or $s_1 \leq s_2$, we have $\frac{2}{2_{s_1}^{*}} + \frac{1}{2_{s_2}^{*}} \leq 1$. The integral $I$ is already finite in the case when $\frac{2}{2_{s_1}^{*}} + \frac{1}{2_{s_2}^{*}} < 1$. Therefore, we consider $\frac{2}{2_{s_1}^{*}} + \frac{1}{2_{s_2}^{*}} = 1$. We apply H\"{o}lder's inequality with exponents $p=\frac{2_{s_1}^{*}}{2},~ q= 2_{s_2}^{*}$ and it follows that
\begin{align*}
    I &\leq \bigg( \int_{\mathbb{R}^{N}}h(x)|u|^{2_{s_1}^{*}}\, \mathrm{d}x \bigg)^{1/p} \bigg(\int_{\mathbb{R}^{N}}h(x)|v|^{2_{s_2}^{*}}\, \mathrm{d}x \bigg)^{1/q}\\
    &\leq \|h\|_{\infty}\bigg( \int_{\mathbb{R}^{N}} |u|^{2_{s_1}^{*}}\, \mathrm{d}x \bigg)^{1/p} \bigg(\int_{\mathbb{R}^{N}} |v|^{2_{s_2}^{*}}\, \mathrm{d}x \bigg)^{1/q},
\end{align*}
since the right side integrals are finite due to the Sobolev embeddings given in \eqref{embeddings} and $h \in L^{\infty}(\mathbb{R}^{N})$, the integral $I$ is also well-defined in this case on the product space $\mathbb{D}$.\\
Finally, we conclude that the right-hand side of \eqref{f2} is finite, and hence the functional $J_\nu$ is well-defined on the product space $\mathbb{D}$.\\
\textbf{(b). The functional $J_\nu$ is $C^1$ on $\mathbb{D}$ :} The functional is given by
\begin{align*}
    J_{\nu}(u,v) &= \frac{1}{2} \|(u,v)\|_{\mathbb{D}}^2 - \frac{1}{2_{s_{1}}^{*}} \|u\|_{2_{s_{1}}^{*}}^{2_{s_{1}}^{*}}  -\frac{1}{2_{s_{2}}^{*}}\|v\|_{2_{s_{2}}^{*}}^{2_{s_{2}}^{*}} - \nu \int_{\mathbb{R}^{N}}h(x)u^2v\, \mathrm{d}x\\
    &= \frac{1}{2} A(u,v) - B(u,v)-\nu I(u,v),
\end{align*} 
where $ A(u,v) = \|(u,v)\|_{\mathbb{D}}^2,~ B(u,v)= \frac{1}{2_{s_{1}}^{*}} \|u\|_{2_{s_{1}}^{*}}^{2_{s_{1}}^{*}}  +\frac{1}{2_{s_{2}}^{*}}\|v\|_{2_{s_{2}}^{*}}^{2_{s_{2}}^{*}} ,~ I(u,v)= \int_{\mathbb{R}^{N}}h(x)u^2v\, \mathrm{d}x$. If $A,B,I \in C^{1}$ on the product space $\mathbb{D}$, then the functional $J_\nu$ is also in $C^1$ on $\mathbb{D}$. It is clear that $A \in C^1$ as it is the square of a norm on $\mathbb{D}$.\\
\textbf{ $B$ is $C^1$ on $\mathbb{D}$:} For every $(\phi, \psi) \in \mathbb{D}$, we have
\begin{equation} \label{b1}
    \frac{B(u+t\phi, v+t \psi)-B(u,v)}{t} = \frac{1}{2_{s_{1}}^{*}}\int_{\mathbb{R}^{N}} \frac{|u+t\phi|^{2_{s_1}^{*}}-|u|^{2_{s_1}^{*}}}{t} \, \mathrm{d}x + \frac{1}{2_{s_{2}}^{*}}\int_{\mathbb{R}^{N}} \frac{|v+t\psi|^{2_{s_2}^{*}}-|v|^{2_{s_2}^{*}}}{t} \, \mathrm{d}x.
\end{equation}
By mean value theorem, there exist $\lambda, \mu \in (0,1)$ such that for $0<|t|<1$, we have
\begin{align*}
    \bigg|\frac{B(u+t\phi, v+t \psi)-B(u,v)}{t} \bigg|& \leq \int_{\mathbb{R}^{N}} |u+\lambda t\phi|^{2_{s_1}^{*}-1}|\phi|\, \mathrm{d}x + \int_{\mathbb{R}^{N}} |v+\mu t\psi|^{2_{s_2}^{*}-1}|\psi|\, \mathrm{d}x\\
    & \leq \int_{\mathbb{R}^{N}} \big(|u|^{2_{s_1}^{*}-1}|\phi| + |\phi|^{2_{s_1}^{*}} \big)\, \mathrm{d}x + \int_{\mathbb{R}^{N}} \big(|v|^{2_{s_2}^{*}-1}|\psi| + |\psi|^{2_{s_2}^{*}} \big)\, \mathrm{d}x.
\end{align*}
The right-side integrals in the last inequality are finite by using the Sobolev embeddings given in \eqref{embeddings}. Therefore, letting $t \rightarrow 0$ in \eqref{b1} and using the dominated convergence theorem we obtain
\begin{align*}
  \lim\limits_{t \rightarrow 0}  \frac{B(u+t\phi, v+t \psi)-B(u,v)}{t} = \int_{\mathbb{R}^{N}} |u|^{2_{s_1}^{*}-2}u \phi \, \mathrm{d}x + \int_{\mathbb{R}^{N}} |v|^{2_{s_2}^{*}-2}v \psi \, \mathrm{d}x.
\end{align*}
Thus we infer that the functional $B$ is Gateaux differentiable on the product space $\mathbb{D}$. Moreover, the Gateaux derivative of $B$ at $(u,v) \in \mathbb{D}$ is given by
\begin{equation} \label{Gateaux}
    \langle B'(u,v)|(\phi, \psi) \rangle = \int_{\mathbb{R}^{N}} |u|^{2_{s_1}^{*}-2}u \phi \, \mathrm{d}x + \int_{\mathbb{R}^{N}} |v|^{2_{s_2}^{*}-2}v \psi \, \mathrm{d}x, \text{ for every }(\phi, \psi) \in \mathbb{D}.
\end{equation}
It remains to check the continuity of the Gateaux derivative to prove that $B$ is Fr\"{e}chet differentiable. We consider a sequence $\{(u_n,v_n)\} \subset \mathbb{D}$ and $(u,v) \in \mathbb{D}$ such that $(u_n,v_n) \rightarrow (u,v)$ strongly in $\mathbb{D}$. Then up to a sub-sequences (still denoted by $(u_n,v_n)$ itself), $(u_n,v_n) \rightarrow (u,v)~\text{a.e. in } \mathbb{R}^N  $. Moreover, using $u_n\rightarrow u$ strongly in $L^{2_{s_1}^{*}}(\mathbb{R}^{N})$ and $v_n\rightarrow v$ strongly in $L^{2_{s_2}^{*}}(\mathbb{R}^{N})$ we have
\begin{align}
  |u_n(x)|\leq U(x) \text{ a.e. in } \mathbb{R}^N \text{ for some } U \in L^{2_{s_1}^{*}}(\mathbb{R}^{N}),\\
   |v_n(x)|\leq V(x) \text{ a.e. in } \mathbb{R}^N \text{ for some } V \in L^{2_{s_2}^{*}}(\mathbb{R}^{N}).
\end{align}
Now for every $(\phi, \psi) \in \mathbb{D}$,
\begin{equation}
    \langle (B'(u_n,v_n)-B'(u,v))|(\phi, \psi) \rangle = \int_{\mathbb{R}^{N}} (|u_n|^{2_{s_1}^{*}-2}u_n-|u|^{2_{s_1}^{*}-2}u) \phi \, \mathrm{d}x + \int_{\mathbb{R}^{N}} (|v_n|^{2_{s_2}^{*}-2}v_n -|v|^{2_{s_2}^{*}-2}v) \psi \, \mathrm{d}x.
\end{equation}
Let us define
\[  E(u) = |u|^{2_{s_1}^{*}-2}u, ~F(v) = |v|^{2_{s_2}^{*}-2}v \text{ and } r_i = \frac{2_{s_i}^{*}}{2_{s_i}^{*}-1},~i=1,2. \]
Clearly, $E(u) \in L^{r_1}(\mathbb{R}^{N})$ and further
\[ |E(u_n)-E(u)|^{r_1} \leq c \big( |E(u_n)|^{r_1} + |E(u_n)|^{r_1}\big) \leq c \big( |U|^{2_{s_1}^{*}} + |u|^{2_{s_1}^{*}} \big) \in L^{1}(\mathbb{R}^{N}),\]
where $c$ is some positive constant varying line by line. By applying dominated convergence theorem, we obtain
\begin{equation}\label{limE}
    \lim\limits_{n \rightarrow \infty} \int_{\mathbb{R}^{N}}|E(u_n)-E(u)|^{r_1}\, \mathrm{d}x = 0.
\end{equation}
 Analogously we also obtain
\begin{equation}\label{limF}
    \lim\limits_{n \rightarrow \infty} \int_{\mathbb{R}^{N}}|F(v_n)-F(v)|^{r_2}\, \mathrm{d}x = 0,
\end{equation}
Consequently, by applying the H\"{o}lder's inequality we have

\begin{align*}
    \big| \langle (B'(u_n,v_n)-B'(u,v))|(\phi, \psi) \rangle\big| &\leq \int_{\mathbb{R}^{N}}|E(u_n)-E(u)| |\phi|\, \mathrm{d}x + \int_{\mathbb{R}^{N}}|F(v_n)-F(v)||\psi|\, \mathrm{d}x\\
    & \leq \|E(u_n)-E(u)\|_{r_1}\|\phi\|_{2_{s_1}^{*}} + \|F(v_n)-F(v)\|_{r_2}\|\psi\|_{2_{s_2}^{*}}.
\end{align*}
This further implies that
\begin{align*}
    \|B'(u_n,v_n)-B'(u,v)\|_{\mathbb{D}^{*}} \leq \|E(u_n)-E(u)\|_{r_1} + \|F(v_n)-F(v)\|_{r_2} \rightarrow 0 \text{ as } n \rightarrow \infty. 
\end{align*}
The above convergence holds due to \eqref{limE} and \eqref{limF}. Thus, we have proved that for every sequence $(u_n,v_n) \rightarrow (u,v)$ in the product space $\mathbb{D}$, there is a subsequence respect to which $B'$ is sequentially continuous. { From this, it is easy to conclude that $B'$ is sequentially continuous in all of $\mathbb{D}^{*}$}. Hence, $B$ is $C^1$ on the product space $\mathbb{D}$.\\
\textbf{$I$ is $C^1$ on $\mathbb{D}$:}
The functional $I$ is given by 
 \[I(u,v)= \int_{\mathbb{R}^{N}}h(x)u^2v\, \mathrm{d}x , \forall ~(u,v) \in \mathbb{D}. \]
For every $(\phi, \psi) \in \mathbb{D}$, we write
 \begin{align*}
    & I(u+t\phi, v+t \psi) - I(u,v)\\
    &= \int_{\mathbb{R}^{N}}h(x)\big((u+t\phi)^{2}(v+t \psi) -u^2v \big)\, \mathrm{d}x\\
     &= \int_{\mathbb{R}^{N}}h(x)\big((u+t\phi)^{2}(v+t \psi) - u^2(v+t \psi)^{} + u^2(v+t \psi)^{}-u^2v \big)\, \mathrm{d}x\\
     &= \int_{\mathbb{R}^{N}}h(x)\big((u+t\phi)^{2}- u^2 \big)(v+t \psi) \, \mathrm{d}x + \int_{\mathbb{R}^{N}}h(x)u^2 \big((v+t \psi)-v \big)\, \mathrm{d}x\\
     &= \int_{\mathbb{R}^{N}}h(x)\big((u+t\phi)^{2}- u^2 \big)(v+t \psi) \, \mathrm{d}x + \int_{\mathbb{R}^{N}}h(x)u^2 t \psi\, \mathrm{d}x\\
 \end{align*}
Further, we have
\begin{align} \label{I1}
\begin{split}
    & \frac{ I(u+t\phi, v+t \psi) - I(u,v)}{t}\\
     &= \int_{\mathbb{R}^{N}}h(x)\bigg(\frac{(u+t\phi)^{2}- u^2}{t} \bigg)(v+t \psi) \, \mathrm{d}x + \int_{\mathbb{R}^{N}}h(x)u^2 \psi\, \mathrm{d}x
     \end{split}
 \end{align}
By mean value theorem, there exist $\lambda \in (0,1)$ such that for $0<|t|<1$, we have
\begin{align*}
    &\bigg|\frac{ I(u+t\phi, v+t \psi) - I(u,v)}{t}\bigg|\\
    &\leq 2 \int_{\mathbb{R}^{N}}h(x) |u+\lambda t\phi| |\phi| |v+t \psi|\, \mathrm{d}x +  \int_{\mathbb{R}^{N}}h(x)|u|^{2}|\psi| \, \mathrm{d}x \\
    &\leq 2 \int_{\mathbb{R}^{N}}h(x)\big( |u||\phi|+|\phi|^{2}\big) |v+t \psi| \, \mathrm{d}x +  \int_{\mathbb{R}^{N}}h(x)|u|^{2}|\psi| \, \mathrm{d}x\\
     &\leq 2 \int_{\mathbb{R}^{N}}h(x)\big( |u||\phi|+|\phi|^{2}\big) |v+ \psi| \, \mathrm{d}x +  \int_{\mathbb{R}^{N}}h(x)|u|^{2}|\psi| \, \mathrm{d}x\\
     &\leq 2 \int_{\mathbb{R}^{N}}h(x) |u| |\phi||v+ \psi| \, \mathrm{d}x+ 2\int_{\mathbb{R}^{N}}h(x)|\phi|^{2} |v+ \psi|\, \mathrm{d}x +
    \int_{\mathbb{R}^{N}}h(x)|u|^{2}|\psi| \, \mathrm{d}x.
\end{align*}
By the assumption $N \leq \min\{6s_1, 6s_2 \}$ and $h \in L^{1}(\mathbb{R}^{N}) \cap L^{\infty}(\mathbb{R}^{N})$, the three integrals in the last inequality are finite. Therefore, letting $t \rightarrow 0$ in \eqref{I1} and using dominated convergence theorem, we have
\begin{align*}
\begin{split}
    &\lim\limits_{t \rightarrow 0} \frac{ I(u+t\phi, v+t \psi) - I(u,v)}{t}\\
     &= 2 \int_{\mathbb{R}^{N}}h(x) u \phi v \, \mathrm{d}x + \int_{\mathbb{R}^{N}}h(x)u^2 \psi\, \mathrm{d}x.
     \end{split}
 \end{align*}
 Thus $I$ is Gateaux differentiable on the product space $\mathbb{D}$ and the Gateaux derivative of $I$ at $(u,v) \in \mathbb{D}$ is defined as
 \begin{align}\label{Gateaux I}
    \langle I'(u,v) | (\phi, \psi) \rangle= 2 \int_{\mathbb{R}^{N}}h(x) u \phi v \, \mathrm{d}x + \int_{\mathbb{R}^{N}}h(x)u^2 \psi\, \mathrm{d}x,
 \end{align}
 for every $(\phi, \psi) \in \mathbb{D}$.\\
 In order to check the Fr\"{e}chet differentiability of $I$, it remains to verify the continuity of the Gateaux derivative of $I$ given by $I'$ in \eqref{Gateaux I}.
 We consider a sequence $\{(u_n,v_n)\} \subset \mathbb{D}$ and $(u,v) \in \mathbb{D}$ such that $(u_n,v_n) \rightarrow (u,v)$ strongly in $\mathbb{D}$. Then up to a sub-sequences (still denoted by $(u_n,v_n)$ itself), $(u_n,v_n) \rightarrow (u,v)~\text{a.e. in } \mathbb{R}^N  $. Moreover, using $u_n\rightarrow u$ strongly in $L^{2_{s_1}^{*}}(\mathbb{R}^{N})$ and $v_n\rightarrow v$ strongly in $L^{2_{s_2}^{*}}(\mathbb{R}^{N})$ we have
\begin{align}
  |u_n(x)|\leq U_1(x) \text{ a.e. in } \mathbb{R}^N \text{ for some } U_1 \in L^{2_{s_1}^{*}}(\mathbb{R}^{N}),\\
   |v_n(x)|\leq V_1(x) \text{ a.e. in } \mathbb{R}^N \text{ for some } V_1 \in L^{2_{s_2}^{*}}(\mathbb{R}^{N}).
\end{align}
Now for every $(\phi, \psi) \in \mathbb{D}$,
\begin{align*}
 \displaystyle   &\langle (I'(u_n,v_n)-I'(u,v))|(\phi, \psi) \rangle \\
    &=2 \int_{\mathbb{R}^{N}} h(x) (u_n v_n-uv) \phi \, \mathrm{d}x +  \int_{\mathbb{R}^{N}} h(x) (u_{n}^2-u^2) \psi \, \mathrm{d}x.\\
    &= 2 \int_{\mathbb{R}^{N}} h(x) \big(u_n-u \big) v_n \phi \, \mathrm{d}x + 2 \int_{\mathbb{R}^{N}} h(x) \big(v_n -v \big) u\phi \, \mathrm{d}x + \int_{\mathbb{R}^{N}} h(x) \big(u_n^{2} -u^{2} \big) \psi \, \mathrm{d}x.
\end{align*}
If $\frac{2}{2_{s_1}^{*}} + \frac{1}{2_{s_2}^{*}} < 1$, we choose $\displaystyle h \in L^{r}(\mathbb{R}^N),~ \displaystyle r = \frac{1}{1-\frac{2}{2_{s_1}^{*}} - \frac{1}{2_{s_2}^{*}}}$ and then applying H\"{o}lder's inequality gives
\begin{align*}
 \displaystyle   &|\langle (I'(u_n,v_n)-I'(u,v))|(\phi, \psi) \rangle |\\
    &\leq 2 \int_{\mathbb{R}^{N}} h(x) |\big(u_n-u \big) v_n \phi| \, \mathrm{d}x + 2 \int_{\mathbb{R}^{N}} h(x)| \big(v_n -v \big) u\phi |\, \mathrm{d}x + \int_{\mathbb{R}^{N}} h(x)| \big(u_n^{2} -u^{2} \big) \psi| \, \mathrm{d}x\\
    &\leq 2  \big\|h(x)\big\|_{r}~ \big\|u_n-u \big\|_{2_{s_1}^{*}} \big\|v_n\big\|_{2_{s_2}^{*}} \big\|\phi\big\|_{2_{s_1}^{*}}  + 2  \big\|h(x)\big\|_{r} \big\|v_n - v \big\|_{2_{s_2}^{*}} \big\|u\big\|_{2_{s_1}^{*}}\big\|\phi\big\|_{2_{s_1}^{*}}  +  \big\|h(x)\big\|_{r} \big\|u_n^2 -u^2 \big\|_{\frac{2_{s_1}^{*}}{2}}  \big\|\psi\big\|_{2_{s_2}^{*}}.
\end{align*}

If $\frac{2}{2_{s_1}^{*}} + \frac{1}{2_{s_2}^{*}} = 1$, we choose $\displaystyle h \in L^{\infty}(\mathbb{R}^N)$ and then applying H\"{o}lder's inequality gives
\begin{align*}
 \displaystyle   &|\langle (I'(u_n,v_n)-I'(u,v))|(\phi, \psi) \rangle |\\
   &\leq 2 \int_{\mathbb{R}^{N}} h(x) |\big(u_n-u \big) v_n \phi| \, \mathrm{d}x + 2 \int_{\mathbb{R}^{N}} h(x)| \big(v_n -v \big) u\phi |\, \mathrm{d}x + \int_{\mathbb{R}^{N}} h(x)| \big(u_n^{2} -u^{2} \big) \psi| \, \mathrm{d}x\\
    &\leq 2  \big\|h(x)\big\|_{\infty}~ \big\|u_n-u \big\|_{2_{s_1}^{*}} \big\|v_n\big\|_{2_{s_2}^{*}} \big\|\phi\big\|_{2_{s_1}^{*}}  + 2  \big\|h(x)\big\|_{\infty} \big\|v_n - v \big\|_{2_{s_2}^{*}} \big\|u\big\|_{2_{s_1}^{*}}\big\|\phi\big\|_{2_{s_1}^{*}}  +  \big\|h(x)\big\|_{\infty} \big\|u_n^2 -u^2 \big\|_{\frac{2_{s_1}^{*}}{2}}  \big\|\psi\big\|_{2_{s_2}^{*}}.
\end{align*}
From both cases, using the boundedness of the sequences $\{u_n\}, \{v_n\}$ in $L^{2_{s_1}^{*}}(\mathbb{R}^{N})$ and $L^{2_{s_2}^{*}}(\mathbb{R}^{N})$ respectively, and $h \in L^{1}(\mathbb{R}^N) \cap L^{\infty}(\mathbb{R}^N)$ we obtain the following
\begin{align} \label{I2}
    \begin{split}
         \displaystyle   & \|(I'(u_n,v_n)-I'(u,v))\|_{\mathbb{D}^{*}} \leq c_1 \big\|u_n -u \big\|_{2_{s_1}^{*}}  + c_2 \big\|v_n - v \big\|_{2_{s_2}^{*}}
       + c_3 \big\|u_n -u \big\|_{\frac{2_{s_1}^{*}}{2}}.
    \end{split}
\end{align}
Let us define
\[  E_1(u) = u, \quad E_2(u) = |u|^2 \text{  and  } F_2(v) = v.\]
We have the following
\[ |E_1(u_n)-E_1(u)|^{2_{s_1}^{*}} \leq c \big( |E_1(u_n)|^{2_{s_1}^{*}} + |E_1(u_)|^{2_{s_1}^{*}}\big) \leq c \big( |U_1|^{2_{s_1}^{*}} + |u|^{2_{s_1}^{*}} \big) \in L^{1}(\mathbb{R}^{N}),\]
where $c$ is some positive constant varying line by line. By applying dominated convergence theorem, we obtain
\begin{equation}\label{limE1}
    \lim\limits_{n \rightarrow \infty} \int_{\mathbb{R}^{N}}|E_1(u_n)-E_1(u)|^{2_{s_1}^{*}}\, \mathrm{d}x = 0.
\end{equation}
Moreover, using a similar set of arguments it holds that 
\begin{equation}\label{limE2}
    \lim\limits_{n \rightarrow \infty} \int_{\mathbb{R}^{N}}|E_2(u_n)-E_2(u)|^{\frac{2_{s_1}^{*}}{2}}\, \mathrm{d}x = 0,
\end{equation}
and 
\begin{equation}\label{limF2}
    \lim\limits_{n \rightarrow \infty} \int_{\mathbb{R}^{N}}|F_2(v_n)-F_2(v)|^{2_{s_2}^{*}}\, \mathrm{d}x = 0,
\end{equation}
Hence, by combining \eqref{I2},\eqref{limE1},\eqref{limE2} and \eqref{limF2} we conclude that
\[ \|(I'(u_n,v_n)-I'(u,v))\|_{\mathbb{D}^{*}} \rightarrow 0 \text{  as  } n \rightarrow \infty. \]
Thus, we have proved that for every sequence $(u_n,v_n) \rightarrow (u,v)$ in the product space $\mathbb{D}$, there is a subsequence respect to which $I'$ is sequentially continuous. { From this, it is easy to conclude that $I'$ is sequentially continuous in all of $\mathbb{D}^{*}$}. Hence, $I$ is $C^1$ on the product space $\mathbb{D}$.\\
Since $A,B$ and $I$ all are $C^1$ functional on the product space $\mathbb{D}$, we conclude that the functional $J_\nu$ is also $C^1$ on $\mathbb{D}$.\\
 For  $(u_0,v_0) \in \mathbb{D}$, the Fr\'{e}chet derivative of $J_\nu$ at $(u,v) \in \mathbb{D}$ is given as follow 
\begin{align*}
     \langle J'_{\nu}(u,v) | (u_0,v_0)\rangle &= \iint_{\mathbb{R}^{2N}} \frac{(u(x)-u(y))(u_0(x)-u_0(y))}{|x-y|^{N+2s_{1}}} \,\mathrm{d}x\mathrm{d}y  \\ &\quad+ \iint_{\mathbb{R}^{2N}} \frac{(v(x)-v(y))(v_0(x)-v_0(y))}{|x-y|^{N+2s_{2}}} \,\mathrm{d}x\mathrm{d}y  - \lambda_1 \int_{\mathbb{R}^{N}} \frac{u\cdot u_0}{|x|^{2s_{1}}}\,\mathrm{d}x - \lambda_2 \int_{\mathbb{R}^{N}} \frac{v \cdot v_0}{|x|^{2s_2}}\,\mathrm{d}x  \\&\quad- \int_{\mathbb{R}^{N}} |u|^{{2^{*}_{s_{1}}}-2} u \cdot u_0 \,\mathrm{d}x
        - \int_{\mathbb{R}^{N}} |v|^{{2^{*}_{s_{2}}}-2} v \cdot v_0 \,\mathrm{d}x\\
       &\quad - 2\nu  \int_{\mathbb{R}^{N}}h(x)u \cdot u_0 v\,\mathrm{d}x
        - \nu  \int_{\mathbb{R}^{N}}h(x) u^{2} v_0 \,\mathrm{d}x,
\end{align*}
where $J'_{\nu}(u,v)$ is the Fr\'{e}chet derivative of $J_\nu$ at $(u,v) \in \mathbb{D}$, and the duality bracket between the product space $\mathbb{D}$ and its dual $\mathbb{D}^*$ is represented as $\langle \cdot,\cdot \rangle$.
From \eqref{energy functional} and for any $\tau>0$, we get
\begin{align} 
%\begin{split}
    J_{\nu}(\tau u,\tau v) &= \frac{\tau^2}{2} \iint_{\mathbb{R}^{2N}} \frac{|u(x)-u(y)|^{2}}{|x-y|^{N+2s_{1}}} \mathrm{d}x\mathrm{d}y + \frac{\tau^2}{2} \iint_{\mathbb{R}^{2N}} \frac{|v(x)-v(y)|^{2}}{|x-y|^{N+2s_{2}}} \mathrm{d}x\mathrm{d}y -  \frac{\lambda_{1} \tau^2}{2} \int_{\mathbb{R}^{N}} \frac{u^{2}~~}{|x|^{2s_{1}}}\mathrm{d}x \notag\\
    &\quad - \frac{\lambda_{2}\tau^2}{2} \int_{\mathbb{R}^{N}} \frac{v^{2}~~}{|x|^{2s_{2}}}\mathrm{d}x - \frac{\tau^{2_{s_{1}}^{*}}}{2_{s_{1}}^{*}}\int_{\mathbb{R}^{N}} |u|^{2_{s_{1}}^{*}}\mathrm{d}x  -\frac{\tau^{2_{s_{2}}^{*}}}{2_{s_{2}}^{*}}\int_{\mathbb{R}^{N}} |v|^{2_{s_{2}}^{*}}\mathrm{d}x - \nu \tau^{3}\int_{\mathbb{R}^{N}}h(x) u^{2} v\,\mathrm{d}x.
%\end{split}
\end{align} 
Clearly, $J_{\nu}(\tau u_{},\tau v_{}) \rightarrow -\infty ~\text{as}~\tau \rightarrow +\infty$ which implies that the functional $J_\nu$ is unbounded from below on $\mathbb{D}$. Here the concept of Nehari manifold plays its role in minimizing the functional $J_{\nu}$ for finding the critical point in $\mathbb{D}$ by using a variational approach. We introduce the Nehari manifold $\mathcal{N}_{\nu}$ associated with the functional $J_\nu$ as
\[\mathcal{N}_{\nu} = \{  (u, v) \in \mathbb{D} \backslash \{(0, 0)\} : \Phi_{\nu}(u,v) = 0    \},\]
where 
\begin{equation} \label{phi function}
    \Phi_{\nu}(u,v) = \langle J'_{\nu}(u,v) | (u,v) \rangle.
\end{equation}
We can see that all the critical points $(u,v) \in \mathbb{D}\backslash \{(0,0)\}$ of the energy functional $J_\nu$ lie in the set $\mathcal{N}_{\nu}$. On Nehari manifolds, we recall some well-known facts for the reader's convenience.

Let $(u,v)$ be an element of the Nehari manifold $\mathcal{N}_{\nu}$. Then the following holds:
\begin{align} \label{equivalent norm}
\begin{split}
    \|(u,v)\|_{\mathbb{D}}^{2} 
    % = [u]_{s_{1}}^{2} - \lambda_1 \int_{\mathbb{R}^{N}}\frac{u^{2}}{|x|^{2s_{1}}}dx + [v]_{s_{2}}^{2}  - \lambda_2 \int_{\mathbb{R}^{N}}\frac{v^{2}}{|x|^{2s_{2}}}dx\\
    = \|u\|_{{2_{s_{1}}^{*}}}^{2_{s_{1}}^{*}} + \|v\|_{{2_{s_{2}}^{*}}}^{2_{s_{2}}^{*}} +3 \nu  \int_{\mathbb{R}^{N}} h(x) u^{2} v \mathrm{d}x.
\end{split}
\end{align}
If we restrict the functional $J_\nu$ on the Nehari manifold $\mathcal{N}_{\nu}$, the functional takes the following form
\begin{align} \label{energy functional on Nehari manifold}
    J_{\nu}|_{\mathcal{N}_{\nu}}(u,v) = \frac{s_{1}}{N} \|u\|_{{2_{s_{1}}^{*}}}^{2_{s_{1}}^{*}} + \frac{s_{2}}{N} \|v\|_{{2_{s_{2}}^{*}}}^{2_{s_{2}}^{*}} +  \frac{\nu}{2}   \int_{\mathbb{R}^{N}} h(x) u^{2} v \,\mathrm{d}x.
\end{align}
Now suppose that $(\tau u,\tau v) \in \mathcal{N}_{\nu}$ for all $(u, v) \in \mathbb{D} \backslash \{(0, 0)\}$. Then using \eqref{equivalent norm} we get the following 
\begin{align} \label{Algebraic equation}
     \|(u,v)\|_{\mathbb{D}}^{2} =  \tau^{2_{s_{1}}^{*} -2} \|u\|_{{2_{s_{1}}^{*}}}^{2_{s_{1}}^{*}} +  \tau^{2_{s_{2}}^{*} -2} \|v\|_{{2_{s_{2}}^{*}}}^{2_{s_{2}}^{*}} + 3\nu  \tau \int_{\mathbb{R}^{N}} h(x) u^{2} v\,\mathrm{d}x.
\end{align}
The above equation is an algebraic equation in $\tau$ and a cautious analysis of equation \eqref{Algebraic equation} shows that this algebraic equation has a unique positive solution. Thus, we can infer that there exists a unique positive $\tau= \tau_{(u,v)}$ such that $(\tau u,\tau v) \in \mathcal{N}_{\nu}$ for all $(u, v) \in \mathbb{D} \backslash \{(0, 0)\}$. By combining (\ref{equivalent norm}) and (\ref{ alpha beta condition}) we obtain that, for any $(u,v) \in \mathcal{N}_{\nu}$ 
\begin{align*} 
       J''_{\nu}(u,v)[u,v]^{2} &= \langle \Phi'_{\nu}(u,v) | (u,v) \rangle  \\
        &= 2 \iint_{\mathbb{R}^{2N}} \frac{|u(x)-u(y)|^{2}}{|x-y|^{N+2s_{1}}} \mathrm{d}x\mathrm{d}y + 2 \iint_{\mathbb{R}^{2N}} \frac{|v(x)-v(y)|^{2}}{|x-y|^{N+2s_{2}}} \mathrm{d}x\mathrm{d}y  
    -  2\lambda_{1} \int_{\mathbb{R}^{N}} \frac{u^{2}}{|x|^{2s_{1}}}\mathrm{d}x\\
    &~~~~ - 2\lambda_{2}\int_{\mathbb{R}^{N}} \frac{v^{2}}{|x|^{2s_{2}}}dx -2_{s_{1}}^{*} \int_{\mathbb{R}^{N}} |u|^{2_{s_{1}}^{*}}\mathrm{d}x 
    -2_{s_{2}}^{*}\int_{\mathbb{R}^{N}} |v|^{2_{s_{2}}^{*}}\mathrm{d}x - 9\nu  \int_{\mathbb{R}^{N}} h(x) u^{2} v\,\mathrm{d}x\\ 
    &= 2 \|(u,v)\|_{\mathbb{D}}^{2}-2_{s_{1}}^{*} \|u\|_{2_{s_{1}}^{*}}^{2_{s_{1}}^{*}} 
    -2_{s_{2}}^{*}\|v\|_{2_{s_{2}}^{*}}^{2_{s_{2}}^{*}} -9 \nu  \int_{\mathbb{R}^{N}} h(x) u^{2} v\,\mathrm{d}x.
    \end{align*} Further calculations give us
    \begin{align} \label{second order derivative}
    %\begin{split}
    J''_{\nu}(u,v)[u,v]^{2}&=- \|(u,v)\|_{\mathbb{D}}^{2} + 3 ( \|u\|_{{2_{s_{1}}^{*}}}^{2_{s_{1}}^{*}}+ \|v\|_{{2_{s_{2}}^{*}}}^{2_{s_{2}}^{*}} )
        - 2_{s_{1}}^{*} \|u\|_{{2_{s_{1}}^{*}}}^{2_{s_{1}}^{*}} - 2_{s_{2}}^{*}\|v\|_{{2_{s_{2}}^{*}}}^{2_{s_{2}}^{*}}\notag\\
       & =- \|(u,v)\|_{\mathbb{D}}^{2} + (3 -2_{s_{1}}^{*} )  \|u\|_{{2_{s_{1}}^{*}}}^{2_{s_{1}}^{*}}+ (3 -2_{s_{2}}^{*})\|v\|_{{2_{s_{2}}^{*}}}^{2_{s_{2}}^{*}} ~< 0 .
          % \end{split}
 \end{align}
Further, by using \eqref{equivalent norm} we can prove the existence of a constant $r_{\nu} > 0$ such that
\begin{align} \label{ norm equal  r}
    \|(u,v)\|_{\mathbb{D}} > r_{\nu} ~~\mbox{for~all}~(u,v) \in \mathcal{N}_{\nu}.
\end{align}
Now by the Lagrange multiplier method, if $(u, v) \in \mathbb{D}$ is a critical point of $J_{\nu}$ on the Nehari manifold $ \mathcal{N}_{\nu}$,  then there exists a $\rho \in \mathbb{R}$ called Lagrange multiplier such that
\[ (J_{\nu}|_{\mathcal{N}_{\nu} } )'(u,v) =  J_{\nu}'(u,v) - \rho \Phi'_{\nu}(u,v) = 0.\]
Thus from the above, we calculate that $\rho \langle \Phi'_{\nu}(u,v)|(u,v) \rangle = \langle J'_{\nu}(u,v)|(u,v) \rangle =0 $. It is clear that $\rho=0$, otherwise the inequality (\ref{second order derivative}) fails to hold, and as a result $J_{\nu}'(u,v) = 0$. Hence, there is a one-to-one correspondence between the critical points of $J_{\nu}$ and the critical points of $J_{\nu}|_{\mathcal{N}_{\nu}}$. The functional $J_{\nu}$ restricted on the Nehari manifold ${\mathcal{N}_{\nu}}$ is also written as
\begin{equation} \label{two one four}
        ( J_{\nu}|_{\mathcal{N}_{\nu}})(u,v) = \frac{1}{6} \|(u,v)\|_{\mathbb{D}}^{2} +  \frac{6s_1-N}{6N} \|u\|_{{2_{s_{1}}^{*}}}^{2_{s_{1}}^{*}}+ \frac{6s_2 -N}{6N}\|v\|_{{2_{s_{2}}^{*}}}^{2_{s_{2}}^{*}}. 
\end{equation} 
Thus, combining the hypotheses (\ref{ alpha beta condition}) and (\ref{ norm equal  r}) with \eqref{two one four}, we deduce
\[J_{\nu}(u,v) >  \frac{1}{6} r_{\nu}^{2} ~~\mbox{for~all}~(u,v) \in \mathcal{N}_{\nu}.\]
We come to the conclusion that the functional $J_\nu$ restricted on $\mathcal{N}_{\nu}$ is bounded from below. Hence, we continue our study to get the solution of \eqref{main problem} by minimizing the energy functional $J_\nu$ on the Nehari manifold $\mathcal{N}_\nu$.
\begin{definition}
If $(u_1,v_1) \in \mathbb{D} \backslash \{(0, 0)\}$ is a critical point of $J_\nu$ over $\mathbb{D}$, then we say that the pair $(u_1,v_1)$ is a bound state solution of \eqref{main problem}. This bound state solution $(u_{1},v_{1})$ is said to be a ground state solution if its energy is minimal among all the bound state solutions i.e.
 \begin{equation} \label{ground state level}
     c_{\nu} = J_{\nu}(u_{1},v_{1}) = \min \{ J_{\nu}(u,v): (u, v) \in \mathbb{D} \backslash \{(0, 0)\} ~\text{and}~ J'_{\nu}(u,v)=0 \}.
 \end{equation}
\end{definition}
